Hydrated anions: From clusters to bulk solution with quasi-chemical theory

The interactions of hydrated ions with solution and interface partners are strong on a chemical energy scale. Here, we test the foremost \textit{ab initio theory} for evaluation of hydration free energies of ions, namely, \textit{quasi-chemical theory} (QCT). We focus on halide anions, but also the hydroxide anion, since they have been outstanding challenges for all theories. QCT is built by identification of inner-shell clusters, separate treatment of those clusters, then integration of those results into the broader-scale solution environment. We exploit a close comparison with mass-spectrometric measurements of ion-hydration equilibria. That theory-experiment comparison is excellent with moderate computational effort here. This agreement reinforces both theory and experiment, and provides a numerically accurate inner-shell contribution to QCT. The inner-shell complexes involving heavier halides display strikingly asymmetric hydration clusters. QCT provides a favorable setting for exploitation of the polarizable continuum model (PCM) when the inner-shell material shields the ion from the outer solution environment. For the asymmetrically hydrated, and less effectively shielded, heavier halide ions, we investigate an inverse procedure in which the inner-shell structures are sampled from readily available AIMD calculations on the bulk solutions. This inverse procedure is a remarkable improvement and our final results are in close agreement with a standard tabulation of hydration free energies. Comparison of anion hydration cluster structures with bulk solutions from AIMD simulations emphasize slight differences: the asymmetries of bulk solution inner-shell structures are moderated, but still present; and inner shells fill to slightly higher average coordination numbers in bulk solution than in clusters.

==> XXXabsract.tex <==
The interactions of hydrated ions with molecular and macromolecular
solution and interface partners are strong on a chemical energy scale.
Here, we recount the foremost \textit{ab initio theory}  for evaluation
of hydration free energies of ions; namely, \textit{quasi-chemical
theory} (QCT).   We focus  on anions, particularly halides but also the
hydroxide anion, since they have been outstanding challenges for all
theories. For example, this work supports understanding
the high selectivity for F$^{-}$ over Cl$^-$ in fluoride-selective ion
channels, despite the identical charge and the size similarity of these
ions.  QCT is built by identification of inner-shell clusters, separate
treatment of those clusters, then integration of those results into the
broader-scale solution environment. Recent work has focused on a close
comparison with mass-spectrometric measurements of ion-hydration
equilibria.  We delineate how \textit{ab initio} molecular dynamics
(AIMD) calculations on ion-hydration clusters, elementary statistical
thermodynamics, and electronic structure calculations on cluster
structures sampled from the AIMD calculations obtain just the free
energies extracted from the cluster experiments.    That
theory-experiment comparison has not been attempted before the work
discussed here, but the agreement is excellent with moderate
computational effort.   This agreement reinforces both theory and
experiment, and provides a numerically accurate inner-shell contribution
to QCT.  The inner-shell complexes involving heavier halides display
strikingly asymmetric hydration clusters. Asymmetric hydration
structures can be problematic for evaluation of the QCT outer-shell
contribution with the polarizable continuum model (PCM).   Nevertheless,
QCT provides a favorable setting for exploitation of PCM when the
inner-shell material shields the ion from the outer  solution
environment. For the more asymmetrically hydrated, and thus less
effectively shielded, heavier halide ions clustered with waters, the PCM
is less satisfactory.  We therefore investigate an inverse procedure in
which the inner-shell structures are sampled from readily available AIMD
calculations on the bulk solutions.  This inverse procedure is a
remarkable improvement; our final results are in close agreement with a
standard tabulation of hydration free energies, and the final composite
results are independent of coordination number on the chemical energy
scale of relevance, as they should be. Finally, comparison of anion
hydration structure in clusters and bulk solutions from AIMD simulations
emphasize some differences: the asymmetries of bulk solution inner-shell
structures are moderated compared with clusters, but still present; and
inner hydration shells fill to slightly higher average coordination
numbers in bulk solution than in clusters.


==> XXXabsract.ttex.tex <==
The interactions of hydrated ions with molecular and macromolecular
solution and interface partners are strong on a chemical energy scale.
Here, we recount the foremost \textit{ab initio theory}  for evaluation
of hydration free energies of ions; namely, \textit{quasi-chemical
theory} (QCT).   We focus  on anions, particularly halides but also the
hydroxide anion, since they have been outstanding challenges for all
theories. For example, this work supports understanding
the high selectivity for F$^{-}$ over Cl$^-$ in fluoride-selective ion
channels, despite the identical charge and the size similarity of these
ions.  QCT is built by identification of inner-shell clusters, separate
treatment of those clusters, then integration of those results into the
broader-scale solution environment. Recent work has focused on a close
comparison with mass-spectrometric measurements of ion-hydration
equilibria.  We delineate how \textit{ab initio} molecular dynamics
(AIMD) calculations on ion-hydration clusters, elementary statistical
thermodynamics, and electronic structure calculations on cluster
structures sampled from the AIMD calculations obtain just the free
energies extracted from the cluster experiments.    That
theory-experiment comparison has not been attempted before the work
discussed here, but the agreement is excellent with moderate
computational effort.   This agreement reinforces both theory and
experiment, and provides a numerically accurate inner-shell contribution
to QCT.  The inner-shell complexes involving heavier halides display
strikingly asymmetric hydration clusters. Asymmetric hydration
structures can be problematic for evaluation of the QCT outer-shell
contribution with the polarizable continuum model (PCM).   Nevertheless,
QCT provides a favorable setting for exploitation of PCM when the
inner-shell material shields the ion from the outer  solution
environment. For the more asymmetrically hydrated, and thus less
effectively shielded, heavier halide ions clustered with waters, the PCM
is less satisfactory.  We therefore investigate an inverse procedure in
which the inner-shell structures are sampled from readily available AIMD
calculations on the bulk solutions.  This inverse procedure is a
remarkable improvement; our final results are in close agreement with a
standard tabulation of hydration free energies, and the final composite
results are independent of coordination number on the chemical energy
scale of relevance, as they should be. Finally, comparison of anion
hydration structure in clusters and bulk solutions from AIMD simulations
emphasize some differences: the asymmetries of bulk solution inner-shell
structures are moderated compared with clusters, but still present; and
inner hydration shells fill to slightly higher average coordination
numbers in bulk solution than in clusters.


==> untitledtext2.tex <==
The interactions of hydrated ions with molecular and
macromolecular solution and interface partners are strong on a chemical energy scale. 
 Here, we recount the foremost \textit{ab initio theory}  for evaluation
of hydration free energies of ions; namely,
\textit{quasi-chemical theory} (QCT).   We focus  on anions,
particularly halides but also the hydroxide anion, since
they have been outstanding challenges for all theories. 
 For example, this work supports understanding
%LRP {\color{red} For example, this work clears the way to understanding
the high selectivity for F$^{-}$ over Cl$^-$ in
fluoride-selective ion channels,
despite the identical charge and the size similarity of these ions.  QCT is built by
identification of inner-shell clusters, separate treatment of those
clusters, then integration of those results into the broader-scale
solution environment. Recent work has focused on a close comparison with
mass-spectrometric measurements of ion-hydration equilibria.  We
delineate how \textit{ab initio} molecular dynamics (AIMD) calculations
on ion-hydration clusters, elementary statistical thermodynamics, and
electronic structure calculations on cluster structures sampled from the
AIMD calculations obtain just the free energies extracted from the
cluster experiments.    That theory-experiment comparison has not been
attempted before the work discussed here, but the agreement is excellent with
moderate computational effort.   This agreement reinforces both theory and
experiment, and provides a numerically accurate inner-shell contribution
to QCT.  The inner-shell complexes involving heavier halides
display strikingly 
asymmetric hydration clusters.  
Asymmetric hydration structures can be
problematic for evaluation 
of the QCT outer-shell contribution with the 
polarizable continuum model (PCM).   Nevertheless, QCT 
provides a favorable 
setting for exploitation of PCM when 
the inner-shell material shields the 
ion from the outer  solution 
environment. For the more asymmetrically hydrated, and thus less effectively 
shielded, heavier halide ions clustered with waters, the PCM is 
less satisfactory.  We therefore 
investigate an inverse procedure in which 
the inner-shell structures are sampled from 
readily available AIMD calculations on the 
bulk solutions.  This inverse procedure
is a remarkable improvement; our 
final results are in close agreement with 
a standard tabulation of hydration free energies, and the 
final composite 
results are independent of 
coordination number on the chemical energy scale of relevance, as they should be. Finally, comparison of anion hydration structure in clusters and bulk solutions from AIMD simulations emphasize some differences: the asymmetries of bulk solution 
inner-shell structures are moderated compared with clusters, but still present; and inner hydration shells fill to slightly higher average coordination numbers in bulk solution than in clusters.

